mmHawkeye: Passive UAV Detection with a COTS mmWave Radar

Small Unmanned Aerial Vehicles (UAVs) are becoming potential threats to security-sensitive areas and personal privacy. A UAV can shoot photos at height, but how to detect such an uninvited intruder is an open problem. This paper presents mmHawkeye, a passive approach for UAV detection with a COTS millimeter wave (mmWave) radar. mmHawkeye doesn't require prior knowledge of the type, motions, and flight trajectory of the UAV, while exploiting the signal feature induced by the UAV's periodic micro-motion (PMM) for long-range accurate detection. The design is therefore effective in dealing with low-SNR and uncertain reflected signals from the UAV. mmHawkeye can further track the UAV's position with dynamic programming and particle filtering, and identify it with a Long Short-Term Memory (LSTM) based detector. We implement mmHawkeye on a commercial mmWave radar and evaluate its performance under varied settings. The experimental results show that mmHawkeye has a detection accuracy of 95.8% and can realize detection at a range up to 80m.

==> chapter/2_Model.tex <==
\section{Theoretical model}
\label{sec:model}
In this section, we first introduce the theoretical model of the PMM feature, which theoretically exists stably during the UAV flight. Then we conduct some preliminary studies to verify the stability of the PMM feature and demonstrate the feasibility of UAV detection and tracking with the PMM feature.

%In this section, we first introduce the theoretical model of the PMM feature, which exists stably during the flight of the UAV and can be used for UAV detection and tracking. Then we conduct some preliminary studies to verify the stability of the PMM feature and demonstrate the feasibility of UAV detection and tracking with PMM feature.

\subsection{PMM Feature}
%When a small UAV is in flight, due to its periodic micro-motion, such as the rotation of its blades, it will induce the periodic and time-varying frequency modulation of the reflected signal, which is called the micro-Doppler effect. The micro-Doppler effect produces a time-varying Doppler frequency shift of the reflected signal and can be used to analyze the micro-motion of the UAV. In order to analyze the micro-Doppler effect, we usually use computationally expensive algorithms such as short-time Fourier transform (STFT) to obtain the joint time-frequency image. However, these algorithms needs to be applied to the corresponding reflected signal at the location of the UAV, which requires the location of the UAV in advance. Therefore, using these algorithms to analyze the micro-Doppler effect for UAV tracking becomes the chicken-and-egg problem.

%To accurate detect and track the UAV under low-quality reflected signals with a mmWave radar, we explore the PMM feature of the flying UAV contained in the reflected signal. When the UAV flies at a certain radial velocity, the corresponding Doppler spectral shift peak will appear in the velocity spectrum of the mmWave radar, called the body velocity peak. In addition, the components of the UAV (such as blades) have periodic micro-motion when the UAV flies. the periodic micro-motion of these components will cause a series of periodic peaks in the velocity spectrum centered on the body velocity peak.

When a small UAV is in flight, due to its radial motion relative to the radar, the flying UAV will induce a certain frequency modulation of the reflected signal, which appears as a spectral shift peak in the Doppler spectrum of the reflected mmWave signal, called the body velocity peak. Meanwhile, the components of the flying UAV (such as rotating blades) have additional periodic micro-motions. These periodic micro-motions will induce the additional periodic and time-varying frequency modulation of the reflected signal, which causes a series of periodic peaks in the Doppler spectrum centered on the body velocity peak. We call them \textbf{the PMM feature of the flying UAV}.


Specifically, a mmWave radar sends \textit{frequency-modulated continuous wave} (FMCW) chirp signals for range estimation and velocity measurement. The frequency difference between the transmitted signal (Tx) and the received signal (Rx) indicates the signal propagation time, which can be used to calculate the distance of the target. Denoting the time-variant distance between the radar and the target by $R(t)$, the transmitted signal and the received signal can be expressed as:
\begin{equation}
\begin{aligned}
    &S_{Tx}(t) = exp[j(2\pi f_ct + \pi Kt^2)] \\
    &S_{Rx}(t) = \alpha S_{Tx}[t - 2R(t)/c]
\end{aligned}
\end{equation}
where $f_c$ and $K$ represent the starting frequency and the chirp slope of the FMCW signal, respectively. $\alpha$ is the propagation loss. By mixing the transmitted signal and the received signal, the \textit{beat frequency signal} $s(t)$ can be obtained as:
\begin{equation}
    s_{bf}(t) = S_{Tx}^*(t)S_{Rx}(t) = \alpha exp[j4\pi(f_c + Kt)R(t)/c]    
\end{equation}
whose phase value indicates the distance $R(t)$.

To obtain the range and the radial velocity of the target, we first conduct a \textit{Range-FFT} operation \cite{ti} on the samples of $s_{bf}(t)$ during a chirp. In this way, the frequency spectrum of $s_{bf}(t)$ is mapped to the range spectrum and the distance of the target can be obtained.

Since the duration of a chirp is around 0.5ms, we can neglect the displacement during this period and focus on the distance change across consecutive chirps. By combining the samples in a certain bin from the Range-FFT results, we can obtain the reflected signal $S(t)$ from the target range bin:
\begin{equation}
    S(t) = \alpha exp[j4\pi f_c R(t)/c]
\end{equation}
If the distance $R(t)$ can be rewritten as $R(t) = R_0 + vt$, $R_0$ and $v$ are the current distance and the radial velocity, respectively. We then perform a \textit{Doppler-FFT} operation \cite{ti} on the samples of $S(t)$ to obtain the Doppler spectrum:
\begin{equation}
    S(f) = \alpha \delta(f - 2vf_c/c)
\end{equation}
where $\delta()$ is the Dirac delta function. The peak of the Doppler spectrum indicates the target velocity. With Range-Doppler-FFT, we can obtain the Range-Doppler spectrum and estimate the range and the velocity of the target.

When the detection target is a UAV, we need to consider not only the body motion of the UAV, but also the impact of these components with periodic micro-motion on the reflected signal. The theoretical model is shown in Fig. \ref{fig:model}. To simplify the understanding, we assume that the UAV's radial velocity relative to the mmWave radar is $v$ and the rotational angular velocity of each blade is $w$. Similarly, considering the small size of the UAV and the long distance between UAV and radar, we also assume that the rotors all exist in a certain range bin and the number of rotors is $Q$. The blades of each rotor can be viewed as consisting of $P$ scattering points. Then we derive the impact of the periodic micro-motion of the blades on the reflected signal. 

Firstly, considering that the distance between UAV and radar is much larger than the distance from the scattering point to the rotor, the distance between the $p$-th scattering point in the $q$-th blade and the mmWave radar $R_{p}(t)$ can be represented as:
\begin{equation}
\begin{aligned}
    &R_{p}(t) = R_{q}(t) + R_{pq}(t) \\
    &R_{q}(t) = R_q + vt, R_{pq}(t) = r_{pq} * cos(\theta_{pq}) * cos(\omega t + \phi_{pq})
\end{aligned}
\end{equation}
where $R_{q}(t)$ represents the distance between the $q$-th rotor and the mmWave radar, $R_q$ is its current distance. the distance between the $p$-th scatter point and the rotor is represented as $r_{pq}$ and its projection to the velocity direction is represented $R_{pq}(t)$. $\theta_{pq}$ is the angle between the blade plane and the velocity direction, and $\phi_{pq}$ is the rotation initial phase of the $p$-th scattering point.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/model.pdf}
    \caption{The theoretical model of PMM feature}
    \label{fig:model}
\end{figure}

We can find that both the radial velocity of the UAV and the blade rotation angular velocity affect the distance between the scattering point and the mmWave radar, which in turn affects the reflected signal. The reflected signal from the scatter point can be expressed as:
\begin{equation}
\begin{aligned}
    S_{pq}(t) = \beta_{pq} exp\{j4\pi f_c [R_{q}(t) + R_{pq}(t)]/c\}
\end{aligned}
\end{equation}
where $\beta_{pq}$ represents the propagation loss, which is related to the propagation distance, the material and roughness of the scattering point, etc. By adding the reflected signals from all scatter points and the body together, we can obtain the reflected signal of a flying UAV:

\begin{equation}
\begin{aligned}
    S(t) = &\alpha exp[j4\pi f_c R(t)/c] + \\
           &\sum_{q=1}^{Q} \sum_{p=1}^{P} \beta_{pq} exp\{j4\pi f_c [R_{q}(t) + R_{pq}(t)]/c\}
\end{aligned}
\end{equation}

If we perform a Doppler-FFT operation on this reflected signal, its Doppler spectrum can be represented as:
\begin{equation}
\begin{aligned}
    S(f) = &\alpha \delta(f - 2vf_c/c) + \\
           &\sum_{q=1}^{Q} \sum_{p=1}^{P} \sum_{m=-\infty}^{+\infty} \gamma_{pq} \delta(f - 2vf_c/c - \omega m/{2\pi})
\end{aligned}
\end{equation}
where $\gamma_{pq}$ represents the frequency loss factor. For more calculation details, the reader can refer to the related work \cite{analysis}. 

With the theoretical derivation of the UAV's Doppler spectrum, we can find that due to the periodic micro-motion of the blades, there will be a periodic series of peaks in the Doppler spectrum. The interval between the peaks is related to the blade rotation velocity, and the amplitudes of the peaks are related to the UAV's characteristics and position relative to the mmWave radar. We call them \textbf{the PMM feature}. Considering that the UAV's blades keep rotating in any flight state, the PMM feature is more stable than other features such as reflection intensity and radial velocity. We can explore this feature for accurate UAV detection and tracking.


\begin{figure}[t]
    \centering
    \subfigure[The flying UAV]{
    \includegraphics[width=0.9\linewidth]{figure/premilinary.pdf}
    }
    \subfigure[The hovering UAV]{
    \includegraphics[width=0.9\linewidth]{figure/premilinary_hover.pdf}
    }
    \caption{The Range-Doppler spectrum of UAV}
    \label{fig:preliminary}
\end{figure}

\subsection{Preliminary Study}
In this section, we conduct some preliminary studies to verify the stability of the UAV's PMM feature and demonstrate the feasibility of UAV detection and tracking with the PMM feature.


\begin{figure*}[t]
     \centering
     \includegraphics[width=0.9\linewidth]{figure/overview.pdf}
     \caption{The overflow of \systemname{}}
     \label{fig:overflow}
\end{figure*}
In our experiments, a commercial mmWave radar (TI IWR6843AOP board) is set on the ground with the antenna array parallel to the ground. The detailed parameter configuration is the same as the subsequent experiments and will be detailed introduced in Section \ref{sec:implementation}. A six-wing UAV with three blades per rotor is steered above the mmWave radar. The UAV is first controlled to ascend at a constant speed of about 1.5m/s from one meter above the mmWave radar. Then the UAV is controlled to hover at a range of about 48m. We randomly select a segment of the reflected signal from these two stages and perform the Range-Doppler-FFT on them. Fig. \ref{fig:preliminary}(a) and Fig. \ref{fig:preliminary}(b) show the Range-Doppler spectrum of the flying UAV and that of the hovering UAV, respectively. %The x-axis is the Doppler frequency of the received signal, the y-axis is the sensing range and the color bar represents the amplitude of the signal.
The results show that (1) Whether the UAV is in flight or hovering, the PMM feature always stably appears in the range bin where it is located. In contrast, the reflection intensity and the radial velocity features are less stable as they are more easily affected by the relative distance and the UAV's motion. (2) When the relative distance of the UAV is far, the PMM feature shrinks and distorts due to the low-quality reflected signal. However, its periodicity still exists stably. Note that the highest peak of the PMM feature in Fig. \ref{fig:preliminary}(b) corresponds to the DC components. In this case, we try to exploit the periodicity of the UAV's PMM feature to achieve accurate detection and tracking.

%As the PMM feature exists stably in the flight of the UAV, we try to use the PMM feature to realize the detection and tracking of non-cooperative UAVs. However, as shown in Fig. \ref{fig:preliminary}, the peak intensity distribution of the PMM feature is related to the UAV's motion and the relative position. It is not stable and difficult to directly apply to our task. The PMM feature further severely shrinks and distorts due to the low-quality reflected signals. In this case, to achieve accurate UAV detection and tracking with the PMM feature, The problem of low-quality reflected signals and unpredictable target motion must be solved.





==> chapter/figure.tex <==
\begin{figure*}[ht]
  \centering 
\begin{minipage}{0.22\textwidth}
\centering 
\includegraphics[width=\textwidth]{figure/trajectory_detection.png}
\caption{The impact of UAV trajectory on detection results}
  \label{fig:trajectory_detect_error}
\end{minipage}
\hspace{0.2cm}
 \begin{minipage}{0.22\textwidth}
 \centering
 \includegraphics[width=\textwidth]{figure/trajectory_range_relative2.png}
  \caption{The impact of UAV trajectory on tracking results}
  \label{fig:trajectory_range_error}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}{0.22\textwidth}
\centering 
\includegraphics[width=\textwidth]{figure/velocity_detection.png}
\caption{The impact of UAV velocity on detection results}
  \label{fig:velocity_detection_error}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}{0.22\textwidth}
\centering 
\includegraphics[width=\textwidth]{figure/velocity_range_relative2.png}
\caption{The impact of UAV velocity on tracking results}
  \label{fig:velocity_range_error}
\end{minipage}
    \vspace{-0.5cm}
\end{figure*}

\begin{figure}[t]
  \centering 
 \begin{minipage}{0.22\textwidth}
 \centering
 \includegraphics[width=\textwidth]{figure/overall_detection.png}
  \caption{The overall performance of UAV detection}
  \label{fig:overall_detection}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}{0.22\textwidth}
\centering 
\includegraphics[width=\textwidth]{figure/overall_range_error_relative2.png}
\caption{The overall performance of UAV tracking}
  \label{fig:overall_range_error}
\end{minipage}
    \vspace{-0.5cm}
\end{figure}

\begin{figure}[t]
  \centering 
 \begin{minipage}{0.22\textwidth}
 \centering
 \includegraphics[width=\textwidth]{figure/material_detection.png}
  \caption{The impact of obstacle material on detection results}
  \label{fig:material_detection_error}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}{0.22\textwidth}
\centering 
\includegraphics[width=\textwidth]{figure/material_range_relative2.png}
\caption{The impact of obstacle material on tracking results}
  \label{fig:material_range_error}
\end{minipage}
    \vspace{-0.5cm}
\end{figure}
